A Method to Assess and Argue for Practical Significance in Software Engineering

A key goal of empirical research in software engineering is to assess practical significance, which answers whether the observed effects of some compared treatments show a relevant difference in practice in realistic scenarios. Even though plenty of standard techniques exist to assess statistical significance, connecting it to practical significance is not straightforward or routinely done; indeed, only a few empirical studies in software engineering assess practical significance in a principled and systematic way. In this paper, we argue that Bayesian data analysis provides suitable tools to assess practical significance rigorously. We demonstrate our claims in a case study comparing different test techniques. The case study's data was previously analyzed (Afzal et al., 2015) using standard techniques focusing on statistical significance. Here, we build a multilevel model of the same data, which we fit and validate using Bayesian techniques. Our method is to apply cumulative prospect theory on top of the statistical model to quantitatively connect our statistical analysis output to a practically meaningful context. This is then the basis both for assessing and arguing for practical significance. Our study demonstrates that Bayesian analysis provides a technically rigorous yet practical framework for empirical software engineering. A substantial side effect is that any uncertainty in the underlying data will be propagated through the statistical model, and its effects on practical significance are made clear. Thus, in combination with cumulative prospect theory, Bayesian analysis supports seamlessly assessing practical significance in an empirical software engineering context, thus potentially clarifying and extending the relevance of research for practitioners.

==> files/3_methodology.tex <==
\section{Methodology}\label{sec:methodology}

The purpose of our evaluation is to verify how our approach contrasts with the current ESE guidelines that use frequentist inference to analyse and report results and observe whether our approach helps practitioners in using the results of an empirical study to make decisions. Our first purpose aims to capture the viewpoint of the researcher and whether the same conclusion can be achieved by both Bayesian and frequentist inference. Therefore, we conduct a re-analysis of an experimental study and then discuss the trade-off between both approaches under the perspective of practical significance. 

The experiment that we re-analyse was published in~\cite{AfzalGITAB2015et} and it evaluates and compares the effectiveness and efficiency of exploratory testing (\ET) and testing with documented test cases (test case based testing, \TST). We will use a subset of that data.

A total of 35 subjects participated in the experiment, such that 12 subjects were classified as less experienced testers (\LE), and 23 were classified as more experienced testers (\ME). The experiment evaluated both techniques using a small, noncritical system as the software under test. The experiment used a $2 \times 2$ (cross-over) design, to avoid learning bias. The effectiveness of each technique was measured by the number of faults the technique found that were classified as true faults, i.e., the number of true positives (\nfaults). The original study found that \ET was significantly better than \TST and that there was no significant difference between less and more experienced testers. Previous studies have also partly confirmed these results, e.g.,~\cite{ItkonenM14exp, Itkonen13ML}.

For the second goal of our evaluation, we interview practitioners about making decisions using the results reported from the experiment. Particularly, we look at credible intervals reported by practitioners when faced with the same decisions based on results shown to them in different formats. For this paper, we compare our approach to the traditional text reported in empirical studies where $p$-values and levels of significance are reported. Our sampling strategy was to select practitioners with roles that handle decision making in software development projects. Therefore, we collected feedback from 22 mid to upper managers at two large companies in Sweden. This is not to be confused with the sample and study investigated during our re-analysis; they are completely disjoint.


==> files/old_8_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Much literature on Bayesian analysis exist, but not all have the clarity that is needed to explain, sometimes, relatively complex concepts. If one would like to read up on the basics of probability and Bayesian statistics we recommend~\cite{jaynes03prob}, for a slightly more in-depth view of Bayesian statistics we recommend~\cite{robert2007bayesian} (in particular Ch.~11 is well worth a read, providing arguments for and against Bayesian statistics). For a hands-on approach to Bayesian analysis, we recommend~\cite{mcelreath15statrethink}; McElreath's book \textit{Statistical Rethinking: A Bayesian Course with Examples in R and Stan} is an example of how seemingly complex issues can be explained beautifully, while at the same time help the reader improve their skills in Bayesian analysis. Finally, there is one book that every researcher should have on their shelf, \textit{Bayesian Data Analysis} by Gelman et al.~\cite{gelman2013bayesian}, which is considered the leading text on Bayesian methods.

In~\cite{ehrlich12MLM}, the authors used multilevel models for assessing communication in global software development, while in~\cite{hassan2017MLM} the authors applied MLMs for studying reviews in an app store. However, both studies used a frequentist approach (maximum likelihood), i.e., not a Bayesian approach.

As far as we can tell, there have only been two studies in software engineering that have applied Bayesian analysis with MLMs~\cite{furia16bayes,ernst18MLM}. In~\cite{furia16bayes}, Furia presents several cases of how Bayesian analysis could be used in computer science and software engineering research. In particular, the aspects of including prior belief\slash knowledge in MLMs are emphasized. In~\cite{ernst18MLM}, on the other hand, the author presents a conceptual replication of an existing study where he shows that MLMs support cross-project comparisons while preserving local context, mainly through the concept of partial pooling,\footnote{Partial pooling takes into account variance between units.} as seen in Bayesian MLMs.

In our case, we will undoubtedly use the concepts of priors and partial pooling---they are after all key to Bayesian analysis and MLMs---however, our end-goal will be to connect out-of-sample predictions, i.e., one of the outputs from Bayesian analysis, to the concept of practical significance, where we make predictions on new data. 

Finally, concerning the combination of MLMs and cumulative prospect theory (CPT), Nilsson et al.~\cite{nilssonRW11cpt} used MLMs to estimate the parameters for CPT in mathematical psychology, i.e., when an experiment has been conducted where CPT is evaluated, what are the parameters estimated from the experiment? As we will see we rely on such estimates for validation purposes concerning practical significance.
